Absent Subsequences in Words

An absent factor of a string $w$ is a string $u$ which does not occur as a contiguous substring (a.k.a. factor) inside $w$. We extend this well-studied notion and define absent subsequences: a string $u$ is an absent subsequence of a string $w$ if $u$ does not occur as subsequence (a.k.a. scattered factor) inside $w$. Of particular interest to us are minimal absent subsequences, i.e., absent subsequences whose every subsequence is not absent, and shortest absent subsequences, i.e., absent subsequences of minimal length. We show a series of combinatorial and algorithmic results regarding these two notions. For instance: we give combinatorial characterisations of the sets of minimal and, respectively, shortest absent subsequences in a word, as well as compact representations of these sets; we show how we can test efficiently if a string is a shortest or minimal absent subsequence in a word, and we give efficient algorithms computing the lexicographically smallest absent subsequence of each kind; also, we show how a data structure for answering shortest absent subsequence-queries for the factors of a given string can be efficiently computed.

==> new_proposition.tex <==
% !TeX spellcheck = en_GB

We can actually show a slightly stronger property: any word which has no proper $\sas$ is a permutation of $A_k$ for a suitable $k$. For the rest of this chapter $\pi$ always denotes a morphism of $\Sigma^\ast$ that acts as a permutation on the letters of $\Sigma$, that is, $\pi$ is a bijection of $\Sigma$ into itself and satisfies $\pi(uv)=\pi(u)\pi(v)$ for all $u,v\in\Sigma^\ast$. For simplicity we call $\pi$ a permutation (of $\Sigma$). In contrast we denote any permutation of integers, e.g. positions of a word, by $\theta$. For illustration let $\pi$ and $\theta$ both denote the permutation that maps $1$ to $2$ and vice versa, then $\pi(1322) = 2311$ and $\theta(1322) = 3122$.

The first observation follows directly.

\begin{lemma}\label[lemma]{perm}
If $\pi$ is a permutation of $\Sigma$ and $w\in\Sigma^*$ then $\pi(v)$ is an $\sas$ of $\pi(w)$ if and only if $v$ is an $\sas$ of $w$.
Hence $|\sas(w)|$ = $|\sas(\pi(w))|$.
\end{lemma}

\begin{proposition}
Let $w\in\Sigma^*$, then $|\sas(w)| = |\mas(w)|$ if and only if there is a permutation $\pi$ such that $\pi(w) = A_{\iota(w)}$.
\end{proposition}

\begin{proof}
The if-part is immediate: $|\sas(w)|=|\sas(\pi(w))|=|\mas(\pi(w))|=|\mas(w)|$ by \cref{propAlternateone}. \par
For the converse let $w\in\Sigma^*$ satisfying $|\sas(w)| = |\mas(w)|$. Firstly assume there is $a\in\Sigma$ such that $|w|_a > \iota(w)$. Then $a^{|w|_a+1}$ is an $\mas$ of $w$ but not an $\sas$ of $w$, a contradiction. So every letter occurs exactly $\iota(w)$ times in $w$ and therefore exactly once in each arch $\ar_w(\ell)$. 
Hence there is a permutation $\pi$ such that $\pi(\ar_w(1)) = v_1$. 
Now assume there is an integer $\ell\leq\iota(w)$ such that $\pi(\ar_w(1)\ar_w(2)\cdots\ar_w(\ell)) \neq A_{\ell}$. Let $k$ be minimal with this property. 
By definition of $\pi$ we have $k>1$ and w.l.o.g we can assume $k$ to be even. 
Then $\pi(\ar_w(k))\neq v_2 = \sigma\cdots 21$, that is we can find two positions $i<j\in\ar_w(k)$ such that $\pi(w[i])<\pi(w[j])$. 
We claim that $u =w[i]^kw[j]^{\iota(w)-k+2}$ is an $\mas$ but not an $\sas$ of $w$.  
We start by checking if $u_1=w[i]^{k-1}w[j]^{\iota(w)-k+2}$ and $u_2=w[i]^kw[j]^{\iota(w)-k+1}$ are subsequences of $w$. 
We have $\pi(\ar_w(k-1))=v_1=12\cdots\sigma$ and $\pi(w[i])<\pi(w[j])$ hence $w[i]w[j]$ occurs in $\ar_w(k-1)$. 
Then $w[i]^{k-1}w[j]$ is a subsequence of $\ar_w(1)\cdots\ar_w(k-1)$ and $w[j]^{\iota(w)-k+1}$ is a subsequence of $\ar_w(k)\cdots\ar_w(\iota(w))$. 
Similarly $w[i]^kw[j]$ is a subsequence of $\ar_w(1)\cdots\ar_w(k)$ and $w[j]^{\iota(w)-k}$ is a subsequence of $\ar_w(k+1)\cdots\ar_w(\iota(w))$. 
So $u_1,u_2$ are subsequences of $w$ and $u$ is an $\mas$ of $w$.
We have $\len u = \iota(w)+2$ and so $u$ is not an $\sas$ of $w$, a contradiction. 
Hence $\pi(\ar_w(1)\cdots\ar_w(\ell))=A_\ell$ holds for all $\ell\leq\iota(w)$ and therefore $\pi(w)=A_{\iota(w)}$.
\end{proof}




